ICE: A General and Validated Energy Complexity Model for Multithreaded Algorithms

Like time complexity models that have significantly contributed to the analysis and development of fast algorithms, energy complexity models for parallel algorithms are desired as crucial means to develop energy efficient algorithms for ubiquitous multicore platforms. Ideal energy complexity models should be validated on real multicore platforms and applicable to a wide range of parallel algorithms. However, existing energy complexity models for parallel algorithms are either theoretical without model validation or algorithm-specific without ability to analyze energy complexity for a wide-range of parallel algorithms. This paper presents a new general validated energy complexity model for parallel (multithreaded) algorithms. The new model abstracts away possible multicore platforms by their static and dynamic energy of computational operations and data access, and derives the energy complexity of a given algorithm from its work, span and I/O complexity. The new model is validated by different sparse matrix vector multiplication (SpMV) algorithms and dense matrix multiplication (matmul) algorithms running on high performance computing (HPC) platforms (e.g., Intel Xeon and Xeon Phi). The new energy complexity model is able to characterize and compare the energy consumption of SpMV and matmul kernels according to three aspects: different algorithms, different input matrix types and different platforms. The prediction of the new model regarding which algorithm consumes more energy with different inputs on different platforms, is confirmed by the experimental results. In order to improve the usability and accuracy of the new model for a wide range of platforms, the platform parameters of ICE model are provided for eleven platforms including HPC, accelerator and embedded platforms.

==> EPEM/reviewer_comments_addressed.tex <==
We would like to thank all reviewers for their valuable and constructive comments. We will address them carefully in the revised version. Please find below our answers to the reviewers’ key questions and comments.

\textbf{General answer}: Please note that the EPEM model is designed for analyzing the energy _complexity_ of algorithms and therefore the model does not give the estimation of absolute energy consumption. The goal of the EPEM model is to answer energy complexity question: “Given two parallel algorithms A and B for a given problem, which algorithm consumes less energy analytically?”. Although complexity models help developing efficient algorithms, there exists a mismatch between the _complexity analysis_ (e.g., time/energy complexity) of an algorithm and the _absolute performance_ (e.g., execution time, energy consumption) of an implementation of the algorithm even for well-established time complexity models (e.g., PRAM) because: 
i) The details of underlying systems (e.g., runtime and architectures) are neglected or abstracted away to keep complexity models simple and suitable for complexity analysis, and 
ii) O-notation represents an _asymptotic upper-bound_ on time/energy complexity. 

PACT 2016 Review #142A

PACT 2016 Review #142B

QUESTIONS:
\begin{itemize}
\item Q: Can you show that the proposed model is better than other currently used?
A: Table 1 Energy Model Summary (page 2) shows how the EPEM model is different from other current models. To the best of our knowledge, the EPEM model is the first energy model that covers all three aspects: 1) ability to analyze the energy complexity of parallel algorithms, 2) applicability to a wide range of algorithms, and 3) model validation. Section 7 Related Work describes how the EPEM model complements the other currently used models.
\item Q: Can you explain how come cache size does not appear in the analysis?
A: Cache size is captured in the EPEM model by the I/O complexity of the algorithm (e.g., Table 10 on page 11). Note that in the EPEM machine model (Section 2.2), cache size Z is a constant and may disappear in the I/O complexity (e.g., O-notation).
\item Q: Can you provide … absolute energy estimate for model and experiment and show how well model matches experiment?
A: Please see the general answer above.
\end{itemize}
COMMENTS:

(b) ..The EPEM model assumes .. the algorithm specifies what executes on each processor. 
	EPEM models does _not_ have that assumption. EPEM model focuses on the energy complexity of algorithms and therefore abstracts away the details of underlying systems (e.g., runtime, architecture)

(c) ..experiments .. CILK.. entails communication.. handled?
	We believe that we should not mix the generality and abstraction of a model for analyzing energy complexity of algorithms (e.g., EPEM model) with the details of a specific system implementation (e.g., work stealing). As defined in the EPEM machine model (Section 2.2), all the inter-core communication is conducted through writing to and reading from the main memory.

The Ideal Cache model (IC).. a parallel algorithm.. more total cache misses than.. sequential algorithm, because of conflicting accesses by distinct processors. Lemma 2.1. uses incorrect assumptions.
	Lemma 2.1 does _not_ state that a parallel algorithm has the same cache misses as the corresponding sequential algorithm. Instead, it states that a parallel algorithm has up to P times more cache misses than the corresponding sequential algorithm, where P is the number of cores. 

.. execution time is not sensitive to memory latency, only to memory bandwidth.. not true..for SpMV.
	In EPEM model, execution time is sensitive to both memory latency (i.e., parameter M in Equation 8 and 10 on page 4) and memory bandwidth (i.e. number of cache line transfers). 

The definition of the static energy of random memory access and random operation does not make much sense….
	The static energy of memory access and operations are necessary to cover all the cases, e.g., when the algorithm is operating only on data in private cache (i.e. no memory access) or writing data from cache to memory without computation.

The model ..assume.. (a) only flop; (..b) ..same amount of time ..energy; (c) .. one operation per cycle. .
	We believe these are misunderstandings: (a) Work complexity is computed in the number of operations (e.g., flops), but I/O complexity is computed in the number of memory accesses;  (b) operations might take different amount of time, and the EPEM model currently use an _average_ dynamic energy for operations (upper-bound on dynamic energy can also be used); (c) an operation is executed with average F cycles (cf. Equation 7, page 4).

.. dynamic power management ..
	As stated at the end of Section 2 (page 4), the algorithms are executed with the highest setting (maximum number of cores and maximum frequency).

.. parallel algorithm .. less static energy consumption than ..sequential algorithm.. nothing is gained.
	The _static_ energy consumption is proportional to the execution time of an algorithm. The sequential algorithm has longer execution time and therefore, it has higher static energy consumption compared to parallel version. The _dynamic_ energy consumption, however, depends on the workload and is similar for both parallel and sequential algorithms.

.. "platform independent energy model..
	Since dynamic energy for a memory access and for an operation are constants, we can always find an upper bound (constant) on these values, which is then used in the platform-independent model. Regarding accuracy, please see the general answer above.

The analysis in Table 5 ..specify the algorithms
	In Table 5, we compare three different SpMV algorithms (i.e., CSR, CSB [8] and CSC as mentioned in the first row). We will make this clear in the revised version.
..memory.. access to L1, L2, l3… in Table 3
	According to the EPEM memory machine model (see section 2.2), only accesses to the memory incur cost. Therefore, we only consider the energy consumption of (random) memory accesses.

The validation experiment .. the number of non-zeros to predict ..more accurate .. than the proposed model.
	The goal of EPEM model is to answer energy complexity question “Given two parallel algorithms A and B for a given problem, which algorithm consumes less energy analytically?”. Only counting the number of non-zero elements of input cannot answer the question since both algorithms should be analyzed using the same input.

matmul.. weak validation..  compares two algorithms.. the same number.. operations, but different.. communication..
	Note that this is I/O complexity rather than the exact amount of communication. Moreover, if two algorithms that have the _same energy complexity_ are used for experimental validation, it is impossible to validate the EPEM model that is designed to address the energy complexity question: "Given two parallel algorithms A and B for a given problem, which algorithm consumes less energy analytically?".                        

PACT 2016 Review #142C

.. the simplicity of the model and a lack of discussion of its inaccuracies that are reported in the experimental evaluation.
	As for well-established time complexity models (e.g., PRAM), the simplicity is desired for the energy complexity models. Therefore, we keep the EPEM models as simple as possible by abstracting away the details of underlying systems (e.g., architecture and run-time). We will add discussion of the model inaccuracies in the revised version. 

QUESTIONS:

Is the assumption that the I/O and computation operations of an algorithm can be completely overlapped overly simplistic?  What impact might this have on the accuracy of the model?
	Pipelining technique in modern architectures enables overlapping computation with memory accesses [17]. This assumption has also been made by another study [10].

What was the role of Choi et. al. and their results in the computation of the system parameters for all of the platforms listed in Table 3?
	From Choi et al. study, we obtain the parameters of the first 9 platforms. The parameters of the two new platforms (Xeon and Xeon Phi) used in the experiments are not available from Choi et al. study. Therefore, we follow the methodology mentioned in Choi et al. study to find their parameters. We will elaborate on this in the revised version.

Why is the ratio computed by the Model a factor of 8 larger than the experimentally evaluated ratio for some of the SpMV inputs? What impact might the simple assumption of overlapped I/O and computation have on this?
In Table 8, what difference was there in the energy use of the two inputs at the points when the model mispredicted?
	Please see the general answer above.

COMMENTS:

.. degree of error and there is insufficient discussion ...
..Figures 3, 4, 8 and 9..Is there any significance in this?
	Please see the general answer above.

.. MATLAB implementation .. as a baseline is needed..  Figure 2 .. redrawing the graph ..
	We will add a citation to [8], which use Matlab as a baseline, as well as add pds-100 to Figure 2 in the revised version.

.. EPEM parameters..used by Choi et al.. detail ..process ..to produce the values.  
	We will add more details on how we obtain the EPEM parameters from Choi et al. study in the revised version. In short, we only duplicate the micro-benchmark code and modify the number of cores according to the new platforms.

In Section 5.7… Figure 5, .. Table 9 and given that at least seven of the 22 (~32%) data sets don't report values for all inputs a log-scale in the y-axis
	We will revise the contribution claim in section 5.7 and Figure 5 according to reviewer’s suggestion. The original claim means the EPEM models can compare different algorithms across _platforms_, which is separate from the results in Table 9 that compare the accuracy of the model across _input types_.

PACT 2016 Review #142D

QUESTIONS:

To verify that the EPEM ..Figure 5 is used to show energy .. when the actual .. ..very close,.. EPEM ..successfully predict the results?

	Please see the general answer above. Even for well-established  time complexity models (e.g., PRAM), it is hard, if not impossible, to predict which of two given algorithms has shorter execution time based on their time _complexity_ (e.g., O-notation) when the actual execution time difference between them are very close.

COMMENTS:

-Only SpMV and Matrix Multiplication benchmarks ..not ..enough.
	Due to the space constraint, we can present only representative applications. SpMV and Matrix Multiplication (Matmul) represent both data-intensive and computation-intensive applications, respectively. For each application, we characterize and compare the energy consumption according to three aspects: different algorithms, different input matrix types and different platforms.

-Figure 5.. not clear ..difficult to conclude...
	We will improve Figure 5 and use log-scale on the y-axis to make it clearer in the revised version.




